ACTNET: end-to-end learning of feature activations and multi-stream aggregation for effective instance image retrieval

We propose a novel CNN architecture called ACTNET for robust instance image retrieval from large-scale datasets. Our key innovation is a learnable activation layer designed to improve the signal-to-noise ratio (SNR) of deep convolutional feature maps. Further, we introduce a controlled multi-stream aggregation, where complementary deep features from different convolutional layers are optimally transformed and balanced using our novel activation layers, before aggregation into a global descriptor. Importantly, the learnable parameters of our activation blocks are explicitly trained, together with the CNN parameters, in an end-to-end manner minimising triplet loss. This means that our network jointly learns the CNN filters and their optimal activation and aggregation for retrieval tasks. To our knowledge, this is the first time parametric functions have been used to control and learn optimal aggregation. We conduct an in-depth experimental study on three non-linear activation functions: Sine-Hyperbolic, Exponential and modified Weibull, showing that while all bring significant gains the Weibull function performs best thanks to its ability to equalise strong activations. The results clearly demonstrate that our ACTNET architecture significantly enhances the discriminative power of deep features, improving significantly over the state-of-the-art retrieval results on all datasets.

==> inv_exp_notes.tex <==
\section{Thoughts on inverse exponential distribution for tensor outputs of DNN conv. layer}

The inputs of the activation layer is typically the tensor output of some convolutional layer of an existing DNN (e.g. ResNet). From data, it was observed that the histogram of values in the this tensor output might follow and exponential distribution (or some other distribution that resembles that). Another possibility is the Lomax distribution. 

In this section, we shall consider the hypothesis that the distribution of each tensor output, for a specific spatial location and channel, follows the exponential distribution.

To this end, let such a single convolutional tensor element be represented as a random variable $\mathbf{A}$. The values that $\mathbf{A}$ can have are positive real numbers, which is consistent with ReLU outputs of convolutional layers. Since we are assuming the exponential distribution, the probability distribution (or cumulative distribution function) for $\mathbf{A}$ is:
\[
F_A(x) = 1 - e^{-\lambda x}
\]

We would like to know how the probability distribution of $\mathbf{A}$ is changed if we were to apply an exponential operation $g(x) = \exp(x/p)$ to the values of that $\mathbf{A}$ can assume. In other words, we want to find the resulting probability density function for the new random variable $\mathbf{Y} = g(\mathbf{A})$.

There are two methods to achieve this, the first is as follows: We note that the CDF for $\mathbf{Y}$ can be defined as:
\[
F_Y(y) = P(\mathbf{Y} \leq y) = P(g(\mathbf{A}\leqy) = R(\mathbf{A} \in R_y)
\]
where $R_y$ is the set of all values of $x$ where $e^{x/p} \leq y$, in otherwords, solving for $x$ in this inequality gives: $y \leq p\ln y$. Thus, $R_y = \{x: x\leq p\ln y, x \geq 0\}$. Importantly, since $x$ is non-negative, this restricts the possible values of $y$ to be greater than 1.

So, the above equation becomes:
\begin{eqnarray*}
F_Y(y) = P\{\mathbf{A} \leq p \ln y\} \\
& = & F_A(p\ln y) \\
& = & 1 - e^{-\lambda p \ln y} \\
& = & 1 - y^{-\lambda p}
\end{eqnarray*}

To obtain the density function, we differentiate the above w.r.t $y$ and noting that $y$ must be greater or equal to 1:
\[
f_Y(y) = \left\{
\begin{array}{cc}
\lambda p y^{-1-\lambda p} &, y \geq 1 \\
0 & \textrm{,otherwise}
\end{array}
\right.
\]
when $y \geq 1$ and 0 otherwise.

To compute the mean of $\mathbf{Y}$, we can simply evaluate the expectation integral:
\[
E[\mathbf{Y}] = \int^{\infty}_{-\infty} yf_y(y) dy
\]
% TODO - put in the evaluation
This gives $1/(\lambda p - 1)$ provided that $\lambda p - 1$ is positive. Otherwise, the mean is infinity.
